Test-Time Zero-Shot Temporal Action Localization

Zero-Shot Temporal Action Localization (ZS-TAL) seeks to identify and locate actions in untrimmed videos unseen during training. Existing ZS-TAL methods involve fine-tuning a model on a large amount of annotated training data. While effective, training-based ZS-TAL approaches assume the availability of labeled data for supervised learning, which can be impractical in some applications. Furthermore, the training process naturally induces a domain bias into the learned model, which may adversely affect the model's generalization ability to arbitrary videos. These considerations prompt us to approach the ZS-TAL problem from a radically novel perspective, relaxing the requirement for training data. To this aim, we introduce a novel method that performs Test-Time adaptation for Temporal Action Localization (T3AL). In a nutshell, T3AL adapts a pre-trained Vision and Language Model (VLM). T3AL operates in three steps. First, a video-level pseudo-label of the action category is computed by aggregating information from the entire video. Then, action localization is performed adopting a novel procedure inspired by self-supervised learning. Finally, frame-level textual descriptions extracted with a state-of-the-art captioning model are employed for refining the action region proposals. We validate the effectiveness of T3AL by conducting experiments on the THUMOS14 and the ActivityNet-v1.3 datasets. Our results demonstrate that T3AL significantly outperforms zero-shot baselines based on state-of-the-art VLMs, confirming the benefit of a test-time adaptation approach.

==> sec/formulation.tex <==
\section{Problem formulation} \label{sec:formulation}
Given an untrimmed video $\video=[{\image}_n]_{n=1}^\numframes$, where $\image$ is the image frame and $\numframes$ is the total number of frames, TAL algorithms aim to localize each temporal window of potential action $\temporalwindow \in \mathbb{R}^2 $ (\ie, indicating the start/end time displacement) and recognize its category $\actionlabel \in \actionclassset$, where $\actionclassset$ is a set of action classes.
Existing literature addressing TAL always involves a dataset $\dataset = \{(\video,~\{(\temporalwindow,~\actionlabel)_i\}_{i=1}^M)\}$ of tuples in the format of a video $\video$ and its labels of $\numpredictions$ action temporal windows $\{(\temporalwindow,\actionlabel)_i\}_{i=1}^M$. $\dataset$ is split into a training set $\trainingset$ for model learning and a test set $\testset$ for model evaluation.

Zero-Shot TAL (ZS-TAL) represents a setup where the model aims to localize and recognize actions of classes that are unseen at training, \ie, the set of action classes in the test set $\testactionclassset$ is disjoint from the set of action classes $\trainactionclassset$ in the training set. Yet, as shown in Sec.~\ref{sec:pre}, state-of-the-art ZS-TAL methods greatly rely on the training set $\trainingset$, resulting in poor generalization capability on other datasets. 

Towards a more practical setup of ZS-TAL, we tackle a new setup, \textit{\ourtask} (\ourtaskshort), where \textit{in-domain} training data is unavailable. 
Specifically, given any test video $\video$, \ourtaskshort~aims to predict $\{\left(\hat{{\temporalwindow}},~\hat{y}\right)_i\}_{i=1}^\numpredictions$, where $\hat{y}\in {\testactionclassset}$ denotes the predicted class label and $\hat{t}\in\mathbb{R}^2$ denotes the predicted start/end time displacements for each one of the $\numpredictions$ temporally located actions. 
Prior to testing, a model for \ourtaskshort~should neither see the action set ${\testactionclassset}$, nor leverage the \textit{in-domain} training data ${\trainingset}$ for adaptation.

==> tables/ablation_oracle50.tex <==
\begin{table}[t]
\small
\centering
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{lccccc|c}
\toprule
\textbf{Oracle} & \multicolumn{6}{c}{\textbf{mAP (\%) $\uparrow$}} \\
                & 0.3 & 0.4 & 0.5 & 0.6 & 0.7 & \textbf{Avg.}  \\ 
\midrule
\rowcolor{ModelGreen}
\methodname     & 20.7 & 14.3 & 8.9 & 5.3 & 2.8 & 10.4 \\
XXX             & 23.6 & 15.9 & 9.8 & 5.7 & 2.9 & 11.6 \\
YYY             & 23.4 & 16.2 & 10.1 & 6.0 & 3.0 & 11.7 \\
ZZZ             & 29.9 & 23.1 & 16.6 & 11.2 & 6.5 & 17.4 \\
WWW             & 38.2 & 29.7 & 21.8 & 14.7 & 8.8 & 22.6 \\
\bottomrule
\end{tabular}
}
\caption{}
\label{oracle}
\end{table}




